Clique counts for network similarity

Counts of small subgraphs, or graphlet counts, are widely applicable to measure graph similarity. Computing graphlet counts can be computationally expensive and may pose obstacles in network analysis. We study the role of cliques in graphlet counts as a method for graph similarity in social networks. Higher-order clustering coefficients and the Pivoter algorithm for exact clique counts are employed

==> table1.tex <==
\begin{table}[ht]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}\hline
 &   COLLAB  &   \makecell{IMDB-\\BINARY}  &   \makecell{IMDB-\\MULTI}  &   \makecell{Github-\\Stargaers}  &   \makecell{Deezer Ego\\Nets}  &   \makecell{Survivor \&   \\ Big Brother} \\\hline
$\mathrm{acc}$  &   59.98\tiny{$\pm$1.57} &   58.03\tiny{$\pm$4.20} &   38.67\tiny{$\pm$2.88} &   51.48\tiny{$\pm$1.13}&   53.59\tiny{$\pm$1.48}&   74.29\tiny{$\pm$7.69}\\\hline
$\mathrm{cc}$  &   63.63\tiny{$\pm$1.92} &   60.55\tiny{$\pm$4.91} &   39.09\tiny{$\pm$2.77}  &55.58\tiny{$\pm$1.06} &   50.07\tiny{$\pm$1.56} &   73.28\tiny{$\pm$6.48}\\\hline
$\mathcal{C}_{4}$ &   {\bf 69.66\tiny{$\pm$1.76}} &   70.06\tiny{$\pm$4.57} &   44.53\tiny{$\pm$3.01} &   54.37\tiny{$\pm$0.86} &   51.59\tiny{$\pm$1.60} &   {\bf 53.64\tiny{$\pm$11.64}}\\
$\mathcal{C}_{5}$ &   64.90\tiny{$\pm$1.87} &   {\bf 70.37\tiny{$\pm$4.11}} &   46.97\tiny{$\pm$3.61} &   54.67\tiny{$\pm$0.94} &   50.96\tiny{$\pm$1.45} &   52.82\tiny{$\pm$10.52}\\
$\mathcal{C}_{6}$ &   67.35\tiny{$\pm$2.11} &   69.91\tiny{$\pm$4.68} &   {\bf 47.44\tiny{$\pm$3.32}} &   54.66\tiny{$\pm$0.88} &   52.38\tiny{$\pm$1.30} &   52.89\tiny{$\pm$12.31}\\
$\mathcal{C}_{7}$ &   {\bf 69.11\tiny{$\pm$1.69}} &   70.76\tiny{$\pm$4.23} &   46.83\tiny{$\pm$3.45} &   54.64\tiny{$\pm$1.19} &   51.49\tiny{$\pm$1.73} &   50.09\tiny{$\pm$11.75}\\
$\mathcal{C}_{8}$ &   68.05\tiny{$\pm$1.88} &   70.50\tiny{$\pm$4.02} &   48.22\tiny{$\pm$3.50} &   54.67\tiny{$\pm$0.95} &   51.40\tiny{$\pm$1.50} &   {\bf 52.30\tiny{$\pm$12.09}}\\
$\mathcal{C}_{9}$ &   67.74\tiny{$\pm$2.03} &   {\bf 71.10\tiny{$\pm$4.05}} &   48.83\tiny{$\pm$3.26} &   54.72\tiny{$\pm$1.02} &   51.30\tiny{$\pm$1.56} &   51.19\tiny{$\pm$11.92}\\
$\mathcal{C}_{10}$ &   68.13\tiny{$\pm$1.91} &   70.68\tiny{$\pm$4.26} &  {\bf 49.41\tiny{$\pm$3.77}} &   54.77\tiny{$\pm$0.91} &   51.40\tiny{$\pm$1.43} &   51.11\tiny{$\pm$11.60}\\
\hline$\mathcal{D}_{4}$ &   67.23\tiny{$\pm$2.09} &   69.16\tiny{$\pm$4.34} &   45.13\tiny{$\pm$3.85} &   58.23\tiny{$\pm$1.25} &   51.16\tiny{$\pm$1.29} &   86.08\tiny{$\pm$6.68}\\
$\mathcal{D}_{5}$ &   68.97\tiny{$\pm$1.90} &   70.75\tiny{$\pm$4.02} &   46.71\tiny{$\pm$4.31} &   58.44\tiny{$\pm$1.12} &   50.64\tiny{$\pm$1.37} &   83.98\tiny{$\pm$7.80}\\
$\mathcal{D}_{6}$ &   68.82\tiny{$\pm$1.93} &   70.46\tiny{$\pm$4.17} &   47.39\tiny{$\pm$3.81} &   58.42\tiny{$\pm$1.56} &   51.39\tiny{$\pm$1.38} &   83.50\tiny{$\pm$6.76}\\
$\mathcal{D}_{7}$ &   68.60\tiny{$\pm$1.77} &   71.53\tiny{$\pm$4.69} &   47.39\tiny{$\pm$3.40} &   58.51\tiny{$\pm$1.38} &   50.98\tiny{$\pm$1.75} &   83.41\tiny{$\pm$6.79}\\
$\mathcal{D}_{8}$ &   68.08\tiny{$\pm$2.10} &   71.10\tiny{$\pm$4.06} &   48.33\tiny{$\pm$3.79} &   58.46\tiny{$\pm$1.32} &   50.94\tiny{$\pm$1.41} &   83.71\tiny{$\pm$7.00}\\
$\mathcal{D}_{9}$ &   68.26\tiny{$\pm$1.95} &   71.41\tiny{$\pm$3.92} &   49.02\tiny{$\pm$4.06} &   58.44\tiny{$\pm$1.51} &   51.11\tiny{$\pm$1.28} &   84.25\tiny{$\pm$7.33}\\
$\mathcal{D}_{10}$ &   68.91\tiny{$\pm$2.15} &   71.51\tiny{$\pm$4.80} &   49.20\tiny{$\pm$3.51} &   58.49\tiny{$\pm$1.01} &   51.05\tiny{$\pm$1.90} &   84.49\tiny{$\pm$6.60}\\
\hline\cite{Morris2020tudataset} &   N/A &   59.8 \tiny{$\pm$ 1.1} &   39.5\tiny{$\pm$ 0.7} &   N/A&   N/A&   N/A \\\hline \end{tabular}
\captionsetup{margin=1cm}
\end{center}
\caption{The prediction accuracy percentage of linear $C$-SVM with $\ell_2$-penalty. 
Each row with $\calC_k$ indicates the results with $\calC_k(G)$ as an input for each network $G$, and each row with $\calD_k$ indicates $\calD_k(G)$ as the input. 
The last row reports the classification results using graphlet kernel from \cite{Morris2020tudataset}, where N/A stands for not available, as they are not recorded in the paper. Due to the small size of the Survivor \&   Big Brother dataset, the standard deviations of the results tend to be larger. 
The bold numbers indicate examples that make $\mathcal{C}_k$ non-unimodal.}
% ; the italic numbers indicate some entries such that $\calC_k$ has higher accuracy than $\calD_k$. }
\label{table: main}
\end{table}
